Multi-Record Web Page Information Extraction From News Websites

In this paper, we focused on the problem of extracting information from web pages containing many records, a task of growing importance in the era of massive web data. Recently, the development of neural network methods has improved the quality of information extraction from web pages. Nevertheless, most of the research and datasets are aimed at studying detailed pages. This has left multi-record "list pages" relatively understudied, despite their widespread presence and practical significance. To address this gap, we created a large-scale, open-access dataset specifically designed for list pages. This is the first dataset for this task in the Russian language. Our dataset contains 13,120 web pages with news lists, significantly exceeding existing datasets in both scale and complexity. Our dataset contains attributes of various types, including optional and multi-valued, providing a realistic representation of real-world list pages. These features make our dataset a valuable resource for studying information extraction from pages containing many records. Furthermore, we proposed our own multi-stage information extraction methods. In this work, we explore and demonstrate several strategies for applying MarkupLM to the specific challenges of multi-record web pages. Our experiments validate the advantages of our methods. By releasing our dataset to the public, we aim to advance the field of information extraction from multi-record pages.

==> Chapters/7_references.tex <==
\begin{thebibliography}{00}
\bibitem{simultaneous} J. Zhu, Z. Nie, J.-R. Wen, B. Zhang, and W.-Y. Ma, “Simultaneous record detection and attribute labeling in web data extraction,” in Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining, Philadelphia PA USA: ACM, Aug. 2006, pp. 494–503. doi: 10.1145/1150402.1150457.
\bibitem{amber} T. Furche, G. Gottlob, G. Grasso, G. Orsi, C. Schallhart, and C. Wang, “AMBER: Automatic Supervision for Multi-Attribute Extraction,” Oct. 22, 2012, arXiv: arXiv:1210.5984. Accessed: Feb. 16, 2024. [Online]. Available: http://arxiv.org/abs/1210.5984
\bibitem{plate} A. San et al., “PLAtE: A Large-scale Dataset for List Page Web Extraction,” Jun. 15, 2023, arXiv: arXiv:2205.12386. Accessed: Oct. 29, 2023. [Online]. Available: http://arxiv.org/abs/2205.12386
\bibitem{markuplm} J. Li, Y. Xu, L. Cui, and F. Wei, “MarkupLM: Pre-training of Text and Markup Language for Visually-rich Document Understanding,” Mar. 11, 2022, arXiv: arXiv:2110.08518. Accessed: Feb. 01, 2024. [Online]. Available: http://arxiv.org/abs/2110.08518
\bibitem{partial_tree_alignment} Y. Zhai and B. Liu, “Web data extraction based on partial tree alignment,” in Proceedings of the 14th international conference on World Wide Web  - WWW ’05, Chiba, Japan: ACM Press, 2005, p. 76. doi: 10.1145/1060745.1060761.
\bibitem{finding_and_extracting} M. Álvarez, A. Pan, J. Raposo, F. Bellas, and F. Cacheda, “Finding and Extracting Data Records from Web Pages,” J Sign Process Syst Sign Image Video Technol, vol. 59, no. 1, pp. 123–137, Apr. 2010, doi: 10.1007/s11265-008-0270-y.
\end{thebibliography}

